InForecaster: Forecasting Influenza Hemagglutinin Mutations Through the Lens of Anomaly Detection

The influenza virus hemagglutinin is an important part of the virus attachment to the host cells. The hemagglutinin proteins are one of the genetic regions of the virus with a high potential for mutations. Due to the importance of predicting mutations in producing effective and low-cost vaccines, solutions that attempt to approach this problem have recently gained a significant attention. A historical record of mutations have been used to train predictive models in such solutions. However, the imbalance between mutations and the preserved proteins is a big challenge for the development of such models that needs to be addressed. Here, we propose to tackle this challenge through anomaly detection (AD). AD is a well-established field in Machine Learning (ML) that tries to distinguish unseen anomalies from the normal patterns using only normal training samples. By considering mutations as the anomalous behavior, we could benefit existing rich solutions in this field that have emerged recently. Such methods also fit the problem setup of extreme imbalance between the number of unmutated vs. mutated training samples. Motivated by this formulation, our method tries to find a compact representation for unmutated samples while forcing anomalies to be separated from the normal ones. This helps the model to learn a shared unique representation between normal training samples as much as possible, which improves the discernibility and detectability of mutated samples from the unmutated ones at the test time. We conduct a large number of experiments on four publicly available datasets, consisting of 3 different hemagglutinin protein datasets, and one SARS-CoV-2 dataset, and show the effectiveness of our method through different standard criteria.

==> Tables/covid_auc.tex <==
\begin{table}[!tbh]
\centering
% fscore
\caption{AUC of predictions on SARS-CoV-2 dataset for $T \in \{5,10\}$. Mean is the average of the results on T for each dataset and model.}
\label{tab:covid_auc}
\begin{tabular}{llccc}
\hline
Dataset & Method &
\multicolumn{1}{c}{T=5} & \multicolumn{1}{c}{T=10} & \multicolumn{1}{c}{Mean} \\ \hline
\multirow{2}{*}{SARS-CoV-2}
& Tempel\cite{yin2020tempel} & 0.9584  & 0.9556 & 0.9570 \\
& Ours   & \textbf{0.9715} & \textbf{0.9653}  & \textbf{0.9684} \\ \hline
\end{tabular}
\end{table}

==> Tables/covid_fscore.tex <==
\begin{table}[!tbh]
\centering
% fscore
\caption{F1-Score of predictions on SARS-CoV-2 dataset for $T \in \{5,10\}$. Mean is the average of the results on T for each dataset and model.}
\label{tab:covid_fscore}
\begin{tabular}{llccc}
\hline
Dataset & Method &
\multicolumn{1}{c}{T=5} & \multicolumn{1}{c}{T=10} & \multicolumn{1}{c}{Mean} \\ \hline
\multirow{2}{*}{SARS-CoV-2}
& Tempel\cite{yin2020tempel} & \textbf{0.4893}  & \textbf{0.4731} & \textbf{0.4812} \\
& Ours   & 0.4727 & 0.3926 & 0.4326 \\ \hline
\end{tabular}
\end{table}

==> Tables/covid_prec.tex <==
\begin{table}[!tbh]
\centering
% fscore
\caption{Precision of predictions on SARS-CoV-2 dataset for $T \in \{5,10\}$. Mean is the average of the results on T for each dataset and model.}
\label{tab:covid_prec}
\begin{tabular}{llccc}
\hline
Dataset & Method &
\multicolumn{1}{c}{T=5} & \multicolumn{1}{c}{T=10} & \multicolumn{1}{c}{Mean} \\ \hline
\multirow{2}{*}{SARS-CoV-2}
& Tempel\cite{yin2020tempel} & \textbf{0.9202}  & 0.9165 & 0.3260 \\
& Ours   & 0.3188 & \textbf{0.7898} & \textbf{0.5543} \\ \hline
\end{tabular}
\end{table}

==> Tables/covid_recall.tex <==
\begin{table}[!tbh]
\centering
% fscore
\caption{Recall of predictions on SARS-CoV-2 dataset for $T \in \{5,10\}$. Mean is the average of the results on T for each dataset and model.}
\label{tab:covid_recall}
\begin{tabular}{llccc}
\hline
Dataset & Method &
\multicolumn{1}{c}{T=5} & \multicolumn{1}{c}{T=10} & \multicolumn{1}{c}{Mean} \\ \hline
\multirow{2}{*}{SARS-CoV-2}
& Tempel\cite{yin2020tempel} & \textbf{0.3333}  & 0.3188 & 0.3260 \\
& Ours   & 0.3188 & \textbf{0.7898} & \textbf{0.5543} \\ \hline
\end{tabular}
\end{table}

==> Template for submissions to Scientific Reports/Figures/H1N1.tex <==
\begin{figure*}[!htb]
          \centering
          \begin{subfigure}[b]{0.55\textwidth}
             \centering
             \includegraphics[width=1\linewidth, scale=0.1]{./Images/H1N1 epitops 1.png}
             \caption*{}
          \end{subfigure}
          \begin{subfigure}[b]{0.55\textwidth}
             \centering
             \includegraphics[width=1\linewidth, scale=0.1]{./Images/H1N1 epitops 2.png}
             \caption*{}
          \end{subfigure}
          \begin{subfigure}[b]{0.55\textwidth}
             \centering
             \includegraphics[width=1\linewidth, scale=0.1]{./Images/H1N1 epitops 3.png}
             \caption*{}
          \end{subfigure}
          \caption{The antigenic structure and the proposed mutations by the current study for H1N1. Symbols represents the proposed alteration by the model in right location (\checkmark), not detected important alteration in antigenic site ($\boxtimes$), and proposed alteration by model that does not reflect any important or high prevalence alteration (\square).}
          \label{fig:mut_h1n1}
\end{figure*}

==> Template for submissions to Scientific Reports/Figures/H3N2.tex <==
\begin{figure*}[!htb]
          \centering
          \begin{subfigure}[b]{0.475\textwidth}
             \centering
             \includegraphics[width=1\linewidth, scale=0.1]{./Images/H3N2 epitop 1.png}
             \caption*{}
          \end{subfigure}
          \begin{subfigure}[b]{0.475\textwidth}
             \centering
             \includegraphics[width=1\linewidth, scale=0.1]{./Images/H3N2 epitop 2.png}
             \caption*{}
          \end{subfigure}
          \begin{subfigure}[b]{0.475\textwidth}
             \centering
             \includegraphics[width=1\linewidth, scale=0.1]{./Images/H3N2 epitop 3.png}
             \caption*{}
          \end{subfigure}
          \begin{subfigure}[b]{0.475\textwidth}
             \centering
             \includegraphics[width=1\linewidth, scale=0.1]{./Images/H3N2 epitop 4.png}
             \caption*{}
          \end{subfigure}
          \caption{The antigenic structure and the proposed mutations by the current study for H3N2. Alignment numbers are set based on the HA gene without the first 16 amino acids of the signal peptide in the figure for illustration of the antigenic locations. While in the assessment by the algorithm, we evaluate this 16 amino acids and represented numbers for locations in table S1.\\
        Symbols represent the proposed alteration by the model in right location (\checkmark), not detected important alteration in antigenic site ($\boxtimes$), and proposed alteration by the model that does not reflect any important or high prevalence alteration (\square).
        }
          \label{fig:mut_h3n2}
        \end{figure*}

==> Template for submissions to Scientific Reports/Figures/ROC_Covid.tex <==
\begin{figure*}[!htb]
  \centering
  \includegraphics[ width=1\linewidth]{./Images/ROC-2.pdf}
  \caption{The ROC curves of our model and Tempel for each experiment on the SARS-CoV-2 dataset.}
  \vspace{180in}
  \label{fig:roc_cov}
\end{figure*}

==> Template for submissions to Scientific Reports/Figures/ROC_Curves.tex <==
\begin{figure*}[!htb]
  \centering
  \includegraphics[trim=3cm 2cm 3cm 3cm,clip, width=1\linewidth]{./Images/ROC.pdf}
  \caption{The ROC curves of our model and Tempel for each experiment on the HA dataset.}
  \vspace{180in}
  \label{fig:roc}
\end{figure*}

==> Template for submissions to Scientific Reports/Figures/Stability.tex <==
\begin{figure*}[!htb]
  \centering
  \includegraphics[trim=3cm 2cm 3cm 2cm,clip, width=1\linewidth]{./Images/Stability.pdf}
  \caption{F1-Score of each experiment over epochs. The validation F1-Score in every epoch is achieved by adjusting the threshold in such a way that maximizes this score on the validation data. Later in the same epoch, this threshold is applied to the test dataset to get the test F1-Score.}
  \label{fig:stab}
\end{figure*}


==> Template for submissions to Scientific Reports/Tables/Auc_Score.tex <==
\begin{table}[!tbh]
\centering
% Recall
\caption{AUC comparison on H1N1, H3N2 and H5N1 datasets for $T \in \{5,10,15\}$. Mean is the average of the results on T for each dataset and model. Our results are significantly better or competative with the SOTA method.}
\label{tab:auc}
\begin{tabular}{llcccc}
\hline
Dataset & Method &
\multicolumn{1}{c}{T=5} & \multicolumn{1}{c}{T=10} & \multicolumn{1}{c}{T=15} & \multicolumn{1}{c}{Mean} \\ \hline
\multirow{2}{*}{H1N1}
& Tempel\cite{yin2020tempel} & 0.8467 & 0.8537 & 0.8455 & 0.8486\\
& Ours   & \textbf{0.9713 $\pm$ 0.0002} & \textbf{0.9713 $\pm$0.00008} & \textbf{0.9715 $\pm$ 0.00015} & \textbf{0.9713}\\ \hline
\multirow{2}{*}{H3N2} & Tempel\cite{yin2020tempel} & 0.8989 & 0.8863 & 0.8884 & 0.8912\\
& Ours   & \textbf{0.9419 $\pm$ 0.00004} & \textbf{0.9419 $\pm$ 0.00004} & \textbf{0.9416 $\pm$ 0.0006} & \textbf{0.9418} \\ \hline
\multirow{2}{*}{H5N1} & Tempel\cite{yin2020tempel} & 0.9657 & 0.9696 & 0.9671 & 0.9674\\
& Ours & \textbf{0.9829 $\pm$ 0.00017} & \textbf{0.983 $\pm$ 0.00021} & \textbf{0.9819 $\pm$ 0.00026} & \textbf{0.9826}\\ \hline
\end{tabular}
\end{table}

==> Template for submissions to Scientific Reports/Tables/F1_Score.tex <==
\begin{table}[!tbh]
\centering
% fscore
\caption{F1-Score of predictions on H1N1, H3N2 and H5N1 datasets for $T \in \{5,10,15\}$. Mean is the average of the results on T for each dataset and model.}
\label{tab:fscore}
\begin{tabular}{llcccc}
\hline
Dataset & Method &
\multicolumn{1}{c}{T=5} & \multicolumn{1}{c}{T=10} & \multicolumn{1}{c}{T=15} & \multicolumn{1}{c}{Mean} \\ \hline
\multirow{2}{*}{H1N1}
& Tempel\cite{yin2020tempel} & \textbf{0.8212}  & \textbf{0.821} & \textbf{0.8213} & \textbf{0.8211}\\
& Ours   & 0.8178 $\pm$ 0.0006 & 0.8176 $\pm$ 0.0004 & 0.81992 $\pm$ 0.0004 & 0.8184\\ \hline
\multirow{2}{*}{H3N2} & Tempel\cite{yin2020tempel} & 0.5957 & 0.5785 & 0.5913 & 0.5885 \\ & Ours   & \textbf{0.5966 $\pm$ 0.0009} & \textbf{0.5979 $\pm$ 0.003} & \textbf{0.60127 $\pm$ 0.001} & \textbf{0.5986} \\ \hline
\multirow{2}{*}{H5N1} & Tempel\cite{yin2020tempel} & 0.5167 & 0.5287 & 0.51722 & 0.5208\\ & Ours & \textbf{0.53083 $\pm$ 0.003} & \textbf{0.5387 $\pm$ 0.001} & \textbf{0.5287 $\pm$ 0.01} & \textbf{0.5327} \\ \hline
% \multirow{2}{*}{H1N1*} & Tempel\cite{yin2020tempel} & 0.413 & \textbf{0.605} & \textbf{0.551} & \textbf{0.523}\\ & Ours & \textbf{0.571 $\pm$ 0.0471} & 0.323 $\pm$ 0.103 & 0.471 $\pm$ 0.098 & 0.455 \\ \hline
\end{tabular}
\end{table}

==> Template for submissions to Scientific Reports/Tables/Precision_Score.tex <==
\begin{table}[!tbh]
\centering
%Precision
\caption{Precision of predictions on H1N1, H3N2 and H5N1 datasets for $T \in \{5,10,15\}$. Mean is the average of the results on T for each dataset and model.}
\label{tab:prec}
\begin{tabular}{llcccc}
\hline
Dataset & Method & \multicolumn{1}{c}{T=5} & \multicolumn{1}{c}{T=10} & \multicolumn{1}{c}{T=15} & \multicolumn{1}{c}{Mean} \\ \hline
\multirow{2}{*}{H1N1} & Tempel\cite{yin2020tempel} & \textbf{0.8423} & \textbf{0.8445} & \textbf{0.8389} & \textbf{0.8419}\\
& Ours   & 0.8330 $\pm$ 0.004 & 0.8292 $\pm$ 0.004 & 0.8333 $\pm$ 0.006 & 0.8318\\ \hline
\multirow{2}{*}{H3N2} & Tempel\cite{yin2020tempel} & \textbf{0.7147} & \textbf{0.7300} & \textbf{0.7358} & \textbf{0.7268}\\
& Ours   & 0.5845 $\pm$ 0.0004 & 0.5694 $\pm$ 0.01 & 0.5786 $\pm$ 0.01 & 0.5775\\ \hline
\multirow{2}{*}{H5N1} & Tempel\cite{yin2020tempel} & \textbf{0.8721} & \textbf{0.8598} & \textbf{0.8791} & \textbf{0.7803}\\
& Ours   & 0.7530 $\pm$ 0.02 & 0.7606 $\pm$ 0.02 & 0.7176 $\pm$ 0.02 & 0.7437 \\ \hline
\end{tabular}
\end{table}

==> Template for submissions to Scientific Reports/Tables/Recall_Score.tex <==
\begin{table}[!tbh]
\centering
% Recall
\caption{Recall of predictions on H1N1, H3N2 and H5N1 datasets for $T \in \{5,10,15\}$. Mean is the average of the results on T for each dataset and model. Our results are competitive with SOTA on these datasets.}
\label{tab:recall}
\begin{tabular}{llcccc}
\hline
Dataset & Method &
\multicolumn{1}{c}{T=5} & \multicolumn{1}{c}{T=10} & \multicolumn{1}{c}{T=15} & \multicolumn{1}{c}{Mean} \\ \hline
\multirow{2}{*}{H1N1}
& Tempel\cite{yin2020tempel} & 0.8012 & 0.7997 & 0.8013 & 0.8007\\
& Ours   & \textbf{0.8033 $\pm$ 0.003} & \textbf{0.8066 $\pm$ 0.003} & \textbf{0.8071  $\pm$ 0.006} & \textbf{0.8056}\\ \hline
\multirow{2}{*}{H3N2} & Tempel\cite{yin2020tempel} & 0.5106 & 0.4793 & 0.4943 & 0.4947\\
& Ours   & \textbf{0.6107 $\pm$ 0.01} & \textbf{0.63305 $\pm$ 0.01} & \textbf{0.62768 $\pm$ 0.02} & \textbf{0.6238} \\ \hline
\multirow{2}{*}{H5N1} & Tempel\cite{yin2020tempel} & 0.3671 & 0.38181 & 0.36643 & 0.3717\\
& Ours & \textbf{0.4158 $\pm$ 0.01} & \textbf{0.4205 $\pm$ 0.009} & \textbf{0.42146 $\pm$ 0.01} & \textbf{0.4192}\\ \hline
\end{tabular}
\end{table}

==> Template for submissions to Scientific Reports/Tables/covid_auc.tex <==
\begin{table}[!tbh]
\centering
% fscore
\caption{AUC of predictions on SARS-CoV-2 dataset for $T \in \{5,10\}$. Mean is the average of the results on T for each dataset and model.}
\label{tab:covid_auc}
\begin{tabular}{llccc}
\hline
Dataset & Method &
\multicolumn{1}{c}{T=5} & \multicolumn{1}{c}{T=10} & \multicolumn{1}{c}{Mean} \\ \hline
\multirow{2}{*}{SARS-CoV-2}
& Tempel\cite{yin2020tempel} & 0.9584  & 0.9556 & 0.9570 \\
& Ours   & \textbf{0.9715} & \textbf{0.9653}  & \textbf{0.9684} \\ \hline
\end{tabular}
\end{table}

==> Template for submissions to Scientific Reports/Tables/covid_fscore.tex <==
\begin{table}[!tbh]
\centering
% fscore
\caption{F1-Score of predictions on SARS-CoV-2 dataset for $T \in \{5,10\}$. Mean is the average of the results on T for each dataset and model.}
\label{tab:covid_fscore}
\begin{tabular}{llccc}
\hline
Dataset & Method &
\multicolumn{1}{c}{T=5} & \multicolumn{1}{c}{T=10} & \multicolumn{1}{c}{Mean} \\ \hline
\multirow{2}{*}{SARS-CoV-2}
& Tempel\cite{yin2020tempel} & \textbf{0.4893}  & \textbf{0.4731} & \textbf{0.4812} \\
& Ours   & 0.4727 & 0.3926 & 0.4326 \\ \hline
\end{tabular}
\end{table}

==> Template for submissions to Scientific Reports/Tables/covid_num.tex <==
\begin{table}[!tbh]
\centering

\caption{Number of sequence samples from January 2020 to December 2020}
\label{tab:covid_num}
\begin{tabular}{lllllllllllll}
\hline
Month & Jan & Feb & Mar & Apr & May & Jun & Jul & Aug & Sep & Oct & Nov & Dec \\ \hline
SARS-CoV-2 & 3   & 116   & 900   & 1500   & 1000   & 960  & 986  & 1031 & 800 & 1146 & 1416 & 900  \\
\hline
\end{tabular}
\end{table}

==> Template for submissions to Scientific Reports/Tables/covid_prec.tex <==
\begin{table}[!tbh]
\centering
% fscore
\caption{Precision of predictions on SARS-CoV-2 dataset for $T \in \{5,10\}$. Mean is the average of the results on T for each dataset and model.}
\label{tab:covid_prec}
\begin{tabular}{llccc}
\hline
Dataset & Method &
\multicolumn{1}{c}{T=5} & \multicolumn{1}{c}{T=10} & \multicolumn{1}{c}{Mean} \\ \hline
\multirow{2}{*}{SARS-CoV-2}
& Tempel\cite{yin2020tempel} & \textbf{0.9202}  & 0.9165 & 0.3260 \\
& Ours   & 0.3188 & \textbf{0.7898} & \textbf{0.5543} \\ \hline
\end{tabular}
\end{table}

==> Template for submissions to Scientific Reports/Tables/covid_recall.tex <==
\begin{table}[!tbh]
\centering
% fscore
\caption{Recall of predictions on SARS-CoV-2 dataset for $T \in \{5,10\}$. Mean is the average of the results on T for each dataset and model.}
\label{tab:covid_recall}
\begin{tabular}{llccc}
\hline
Dataset & Method &
\multicolumn{1}{c}{T=5} & \multicolumn{1}{c}{T=10} & \multicolumn{1}{c}{Mean} \\ \hline
\multirow{2}{*}{SARS-CoV-2}
& Tempel\cite{yin2020tempel} & \textbf{0.3333}  & 0.3188 & 0.3260 \\
& Ours   & 0.3188 & \textbf{0.7898} & \textbf{0.5543} \\ \hline
\end{tabular}
\end{table}

==> Template for submissions to Scientific Reports/Tables/last.tex <==
\begin{figure}[!htb]
\begingroup
  \footnotesize 
  \setlength\LTleft{15pt}%
  \setlength\LTright{15pt}%
  \centering 
  \begin{longtable}{@{\extracolsep{\fill}}|c |c| c| c| c| c| c| c| c@{}|}
     \caption{The model's results for different possible amino acid alteration locations.\label{tab:other_methods}}\\
    \hline\hline %inserts double horizontal lines
  Virus type & Mutation &\multicolumn{3}{c}{Current study} & & \multicolumn{3}{c}{Tempel} \\
 % & location &  & & &\\
  \midrule
  & & Mutation & Mutation & Mutation^{*} & & Mutation & Mutation & Mutation^{*}\\
  & & Recall & Precision &  & & Recall & Precision &  \\
  \cmidrule{3-5} \cmidrule{7-9}
  \multirow{3}{*}{H1N1(T5, T10, T15)} & 69 & 0.92 & 0.97 & Y & & 0.95 & 0.97 & Y\\
  & 70 & 0.93 & 0.95 & N & & 0.9 & 0.95 & N\\
  & 85 & 0.89 & 0.95 & Y & & 0.89 & 0.97 & Y\\
  & 95 & 0.97 & 1 & N & & 0.97 & 1 & N\\
  & 132 & 0.93 & 0.89 & N & & 0.95 & 0.9 & N\\
  & 139 & 0.89 & 0.95 & N & & 0.95 & 1 & N\\
  & 140 & 0.91 & 0.91 & N & & 0.89 & 0.91 & N\\
  & 142 & 0.92 & 1 & N & & 0.92 & 1 & N\\
  & 152 & 0.91 & 1 & Y & & 0.93 & 1 & N\\
  & 165 & - & - & - & & 0.95 & 0.97 & Y\\
  & 166 & 0.84 & 0.97 & N & & - & - & -\\
  & 168 & 0.97 & 0.95 & N & & 0.9 & 0.95 & N\\
  & 170 & 0.88 & 0.97 & Y & & 0.88 & 0.97 & Y\\
  & 174 & - & - & - & & 0.9 & 0.92 & Y\\
  & 205 & 0.95 & 0.93 & Y & & 0.93 & 0.93 & Y\\
  & 226 & 0.9 & 0.97 & Y & & 0.89 & 0.95 & Y\\
  & 253 & 0.93 & 0.97 & Y & & 0.93 & 0.97 & Y\\
  & 276 & 0.86 & 0.97 & Y & & 0.9 & 0.97 & Y\\
  \midrule
    \multirow{3}{*}{H3N2(T5, T10, T15)} & 44 & 0.75 & 0.5 & N & & 1 & 1 & N\\
  & 88 & - & - & - & & 0.84 & 1 & N\\
  & 177 & 1 & 0.83 & N & & - & - & -\\
  & 193 & 1 & 0.85 & Y & & - & - & -\\
  & 197 & 1 & 0.85 & Y & & 0.5 & 1 & Y\\
  & 198 & 0.58 & 0.31 & Y & & 0.58 & 0.77 & Y\\
  & 201 & 0.5 & 0.28 & N & & 0.25 & 0.5 & N\\
  & 203 & 0.66 & 0.77 & N & & 0.41 & 1 & N\\
  & 207 & 1 & 0.8 & N & & 0.5 & 1 & N\\
  & 208 & 0.87 & 0.85 & N & & 0.57 & 1 & N\\
  & 209 & 0.75 & 0.6 & N & & 0.5 & 1 & N\\
  & 212 & 0.45 & 0.62 & Y & & 0.36 & 1 & Y\\
  & 213 & 0.46 & 0.8 & N & & 0.28 & 1 & N\\
  & 214 & 0.57 & 0.75 & N & & 0.3 & 1 & N\\
  & 215 & 0.8 & 0.5 & N & & 0.4 & 0.67 & N\\
  & 216 & 0.69 & 0.5 & N & & 0.53 & 1 & N\\
  & 217 & 0.9 & 0.76 & N & & 0.81 & 1 & N\\
  & 218 & 0.95 & 0.87 & N & & 0.45 & 1 & N\\
  \midrule
   
      \multirow{3}{*}{H5N1(T5, T10, T15)} & 82 & 1 & 1 & Y & & 1 & 1 & Y\\
  & 91 & 1 & 1 & N & & 1 & 1 & N\\
  & 116 & 1 & 1 & Y & & 1 & 1 & Y\\
  & 118 & - & - & - & & 1 & 1 & N\\
  & 130 & - & - & - & & 1 & 1 & Y\\
  & 152 & 1 & 1 & Y & & 1 & 1 & Y\\
  & 162 & 1 & 1 & N & & 1 & 1 & N\\
  & 163 & 1 & 1 & N & & 1 & 1 & N\\
  & 165 & 1 & 0.5 & N & & - & - & -\\
  & 166 & 1 & 1 & Y & & 1 & 1 & Y\\
  & 179 & 0.5 & 1 & Y & & - & - & -\\
  & 172 & 0.5 & 1 & Y & & - & - & -\\
  & 182 & 0.25 & 0.66 & N & & 0.25 & 0.67 & N\\
  & 185 & 1 & 1 & Y & & 0.5 & 1 & Y\\
  & 193 & 1 & 1 & N & & 1 & 1 & N\\
  & 205 & 1 & 1 & Y & & 1 & 1 & Y\\
  & 242 & 1 & 1 & Y & & 1 & 1 & Y\\
  \midrule
  \multicolumn{9}{c}{Y: Yes, N: No, *: No, does not express that there is no mutation in all of the available data} \\
  \multicolumn{9}{c}{for 2016. Only that the mutations are not present in the current random sampling.} \\
    \hline %inserts single line
  \end{longtable}
\endgroup
\end{figure}

==> Template for submissions to Scientific Reports/Tables/other_models.tex <==
\begin{table}[!tbh]
\centering

\caption{Precision, recall and F1-score on H1N1, H3N2 and H5N1 datasets for $T \in \{5,10,15\}$. Results are for four different methods including ARAE, GOAD, ESAD and original DeepSAD.}
\label{tab:2}
\begin{tabular}{@{}lllllllllllll@{}}
  \toprule
  Dataset & Model &\multicolumn{3}{c}{Precision} & & \multicolumn{3}{c}{Recall} & &\multicolumn{3}{c}{F1-score} \\
  \midrule
   & & T=5 & T=10 & T=15 & & T=5 & T=10 & T=15 & & T=5 & T=10 & T=15 \\
  \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13}
  \multirow{3}{*}{H1N1} & ARAE & 0.162 & 0.171 & 0.181 & & 0.472 & 0.501 & 0.532 & & 0.241& 0.255& 0.270\\
  & GOAD & 0.124 & 0.132 & 0.190 & & 0.361 & 0.391 & 0.555 & & 0.185& 0.197& 0.283\\
  & ESAD & 0.384 & 0.406 & 0.419 & & 0.570 & 0.573 & 0.589 & & 0.459& 0.475& 0.490\\
  & DeepSAD & 0.294 & 0.318 & 0.322 & & 0.497 & 0.477 & 0.478 & & 0.369 & 0.382 & 0.385\\
  \midrule
  \multirow{3}{*}{H3N2} & ARAE & 0.171 & 0.210 & 0.219 & & 0.498 & 0.611 & 0.639 & & 0.255& 0.313& 0.326\\
  & GOAD & 0.152 & 0.178 & 0.190 & & 0.444 & 0.568 & 0.555 & & 0.226& 0.271& 0.283\\
  & ESAD & 0.279 & 0.290 & 0.331 & & 0.499 & 0.511 & 0.509 & & 0.358& 0.370 & 0.401\\
  & DeepSAD & 0.343 & 0.359 & 0.392 & & 0.536 & 0.540 & 0.565 & & 0.418 & 0.431 & 0.463\\
  \midrule
  \multirow{3}{*}{H5N1} & ARAE & 0.175 & 0.187 & 0.186 & & 0.488 & 0.505 & 0.512 & & 0.258& 0.273& 0.273\\
  & GOAD & 0.217 & 0.238 & 0.235 & & 0.538 & 0.566 & 0.569 & & 0.309& 0.335& 0.333\\
  & ESAD & 0.347 & 0.371 & 0.350 & & 0.568 & 0.538 & 0.482 & & 0.431& 0.439 & 0.406\\
  & DeepSAD & 0.418 & 0.453 & 0.471 & & 0.620 & 0.617 & 0.619 & & 0.499 & 0.522 & 0.535\\
  \bottomrule
\end{tabular}
\end{table}

==> Template for submissions to Scientific Reports/Tables/transformer.tex <==
\begin{table}[!tbh]
\centering

\caption{Recall, F1-score and AUC on H1N1, H3N2 and H5N1 datasets for $T \in \{5,10,15\}$. Results are for The Transformer Network and Tempel}
\label{tab:transformer}
\begin{tabular}{@{}lllllllllllll@{}}
  \toprule
  Dataset & Method &\multicolumn{3}{c}{Recall} & & \multicolumn{3}{c}{F1-score} & &\multicolumn{3}{c}{AUC} \\
  \midrule
  & & 5 & 10 & 15 & & 5 & 10 & 15 & & 5 & 10 & 15 \\
  \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13}
  \multirow{2}{*}{H1N1} & Tempel & 0.80128 & 0.79972 & 0.80137 & & 0.82128 & 0.82102 & \textbf{0.82138} & & 0.84677 & 0.85376 & 0.84551\\
     & Transformer & \textbf{0.8024} & \textbf{0.80137} & \textbf{0.80432} & & \textbf{0.82151} & \textbf{0.8218} & 0.81867 & & \textbf{0.9717} & \textbf{0.9711} & \textbf{0.96935}\\ \hline
  \midrule
  \multirow{2}{*}{H3N2} & Tempel & 0.51069 & 0.479381 & 0.49432 & & 0.59571 & 0.57859 & \textbf{0.59137} & & 0.89896 & 0.88632 & 0.88847\\
     & Transformer & \textbf{0.63373} & \textbf{0.632757} & \textbf{0.5949} & & \textbf{0.6196} & \textbf{0.61002} & 0.5902 & & \textbf{0.9445} & \textbf{0.9354} & \textbf{0.91917}\\ \hline
  \midrule
  \multirow{2}{*}{H5N1} & Tempel & 0.3671 & 0.38181 & 0.36643 & & 0.5167 & \textbf{0.52878} & \textbf{0.51722} & & 0.96572 & 0.9696 & 0.96715\\
     & Transformer & \textbf{0.38083} & \textbf{0.43426} & \textbf{0.42167} & & \textbf{0.5174} & 0.48174 & 0.49658 & & \textbf{0.98874} & \textbf{0.97638} & \textbf{0.97603}\\ \hline
  \bottomrule
\end{tabular}
\end{table}
